Neural Image Representations for Multi-Image Fusion and Layer Separation

We propose a framework for aligning and fusing multiple images into a single view using neural image representations (NIRs), also known as implicit or coordinate-based neural representations. Our framework targets burst images that exhibit camera ego motion and potential changes in the scene. We describe different strategies for alignment depending on the nature of the scene motion -- namely, perspective planar (i.e., homography), optical flow with minimal scene change, and optical flow with notable occlusion and disocclusion. With the neural image representation, our framework effectively combines multiple inputs into a single canonical view without the need for selecting one of the images as a reference frame. We demonstrate how to use this multi-frame fusion framework for various layer separation tasks. The code and results are available at https://shnnam.github.io/research/nir.

==> figures/ablation_rain.tex <==
\begin{figure*}
    \centering
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{ccccccccc}
    \includegraphics[width=0.19\textwidth]{figures/ablation/rain/input.png} & \includegraphics[trim=0 0 176 0,clip,width=0.095\textwidth]{figures/ablation/rain/scene_occlfree.png} & \includegraphics[trim=176 0 0 0,clip,width=0.095\textwidth]{figures/ablation/rain/rain_occlfree.png} & \includegraphics[trim=0 0 176 0,clip,width=0.095\textwidth]{figures/ablation/rain/scene_nointerf.png} & \includegraphics[trim=176 0 0 0,clip,width=0.095\textwidth]{figures/ablation/rain/rain_nointerf.png} & \includegraphics[trim=0 0 176 0,clip,width=0.095\textwidth]{figures/ablation/rain/scene_notvflow.png} & \includegraphics[trim=176 0 0 0,clip,width=0.095\textwidth]{figures/ablation/rain/rain_notvflow.png} & \includegraphics[trim=0 0 176 0,clip,width=0.095\textwidth]{figures/ablation/rain/scene_l02.png} & \includegraphics[trim=176 0 0 0,clip,width=0.095\textwidth]{figures/ablation/rain/rain_l02.png} \\
    % & \includegraphics[trim=0 0 176 0,clip,width=0.095\textwidth]{figures/ablation/rain/flow_occlfree.png} & \includegraphics[trim=176 0 0 0,clip,width=0.095\textwidth]{figures/ablation/rain/w_occlfree.png} & \includegraphics[trim=0 0 176 0,clip,width=0.095\textwidth]{figures/ablation/rain/flow_l0002.png} & \includegraphics[trim=176 0 0 0,clip,width=0.095\textwidth]{figures/ablation/rain/w_l0002.png} & \includegraphics[trim=0 0 176 0,clip,width=0.095\textwidth]{figures/ablation/rain/flow_l02.png} & \includegraphics[trim=176 0 0 0,clip,width=0.095\textwidth]{figures/ablation/rain/w_l02.png} & \includegraphics[trim=0 0 176 0,clip,width=0.095\textwidth]{figures/ablation/rain/flow_l2.png} & \includegraphics[trim=176 0 0 0,clip,width=0.095\textwidth]{figures/ablation/rain/w_l2.png} \\
    {\small Input} & \multicolumn{2}{c}{\small Occlusion-free} & \multicolumn{2}{c}{\small Occlusion-aware} & \multicolumn{2}{c}{\small Occlusion-aware} & \multicolumn{2}{c}{\small Occlusion-aware} \\
    & & & \multicolumn{2}{c}{\small (Without $\lossftwo$)} & \multicolumn{2}{c}{\small (Without $\lossTVFlow$)} & \multicolumn{2}{c}{\small (Full objective)} \\
    & \multicolumn{2}{c}{\small PSNR: 29.52} & \multicolumn{2}{c}{\small PSNR: 28.73} & \multicolumn{2}{c}{\small PSNR: 30.78} & \multicolumn{2}{c}{\small PSNR: \textbf{33.81}}
    % & \multicolumn{2}{c}{\small SSIM: 0.713} & \multicolumn{2}{c}{\small SSIM: 0.732} & \multicolumn{2}{c}{\small SSIM: 0.710} & \multicolumn{2}{c}{\small SSIM: 0.851}
    \end{tabular}
    \caption{Ablation study on the occlusion-aware flow-based neural representations. For each experiment, the left and right column show the underlying scene and rain streaks, respectively.}
    \label{fig:ablation_rain}
\end{figure*}

==> figures/ablation_reflection.tex <==
\begin{figure}
    \centering
    {
    \setlength{\tabcolsep}{1pt}
    \renewcommand{\arraystretch}{0.5}
    \begin{tabular}{ccc}
    \multirow{2}{*}[0.55in]{\includegraphics[width=0.12\textwidth]{figures/ablation/reflection/input.jpg}} & \includegraphics[trim=0 550 0 0,clip,width=0.12\textwidth]{figures/ablation/reflection/scene_nointerf.jpg} & \includegraphics[trim=0 550 0 0,clip,width=0.12\textwidth]{figures/ablation/reflection/scene_notvflow.jpg} \\
    & \includegraphics[trim=0 0 0 550,clip,width=0.12\textwidth]{figures/ablation/reflection/reflection_nointerf.jpg} & \includegraphics[trim=0 0 0 550,clip,width=0.12\textwidth]{figures/ablation/reflection/reflection_notvflow.jpg} \\
    {\small Input} & {\small Without $\lossftwo$} & {\small Without $\lossTVFlow$} \\
    & \includegraphics[trim=0 550 0 0,clip,width=0.12\textwidth]{figures/ablation/reflection/scene_noexcl.jpg} & \includegraphics[trim=0 550 0 0,clip,width=0.12\textwidth]{figures/ablation/reflection/scene.jpg} \\
    & \includegraphics[trim=0 0 0 550,clip,width=0.12\textwidth]{figures/ablation/reflection/reflection_noexcl.jpg} & \includegraphics[trim=0 0 0 550,clip,width=0.12\textwidth]{figures/ablation/reflection/reflection.jpg} \\
    & {\small Without $\lossExcl$} & {\small Full objective}
    \end{tabular}
    }
    \caption{Ablation study of loss functions on reflection removal. The top and bottom images show the background and reflection layer, respectively.}
    \label{fig:ablation_reflection}
\end{figure}

==> figures/ablation_w.tex <==
\begin{figure}
    \centering
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{cc}
    % \includegraphics[width=0.2\textwidth]{figures/ablation/rain/input.png} & \includegraphics[width=0.2\textwidth]{figures/ablation/rain/gt.png} \\
    % {\small Input} & {\small Ground Truth} \\
    \includegraphics[width=0.2\textwidth]{figures/ablation/rain/scene_occlfree.png} & \includegraphics[width=0.2\textwidth]{figures/ablation/rain/scene_l02.png} \\
    {\small Without $w$} & {\small With $w$} \\
    {\small PSNR: 20.42} & {\small PSNR: 24.15}
    \end{tabular}
    \caption{Ablation study on $w$. We show PSNRs of two outputs using the synthetic dataset RainSynLight25~\cite{Liu:2018:RainSyn}, and omit the input and ground truth images.}
    \label{fig:ablation_w}
\end{figure}

==> tables/reflection.tex <==
\begin{table}
\begin{center}
\begin{tabular}{lcccc}
\toprule
Method & Type & PSNR & SSIM & NCC \\
\hline
Li and Brown & Optim. & 17.12 & 0.6367 & 0.6673 \\
Guo~\etal & Optim. & 14.58 & 0.5077 & 0.5802 \\
Alayrac~\etal & CNN & 23.62 & 0.7867 & 0.9023 \\
Liu~\etal & CNN & 26.57 & 0.8676 & 0.9380 \\
Ours & Optim. & 15.13 & 0.6431 & 0.7045 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Quantitative evaluation on reflection removal.}
\label{table:reflection}
\end{table}
